One Fabrication Is Enough: A Fake News Article Changes the Forecasts of LLM Forecasting Systems

LLMs are increasingly used for forecasting, and the best forecasting systems retrieve news as evidence to strengthen their predictions. This also opens them to attack. We study the weakest attacker of this kind, who knows only the forecasting question and publishes fabricated news articles, with no access to the model, the retriever or its queries. We evaluate how far this attack reaches on stock questions and real prediction-market questions. Once the article is in the model's context, it reverses 74% to 82% of the forecasts that opposed it, on every frontier model we tested. The model cannot verify the fabrication and follows it anyway. Retrieval is the attack's entry point, and the systems built to retrieve well are the most exposed: the architectures of two leading deployed forecasting systems, whose agents search for every related article, retrieve the fabricated one in about 90% of runs. Accuracy cannot reveal this harm: the attacked forecaster is right when the attacker's direction turns out right and wrong otherwise, so its average accuracy barely changes while its forecasts follow the attacker's guess. We also propose a second attacker, who publishes two articles that argue opposite directions to make the forecaster unsure. The model does not hedge; it returns a confident forecast in a direction the attacker no longer controls. We then evaluate the two strongest published retrieval-time defenses, passage filtering and partitioned retrieval. Each stops the one-article attack but is bypassed by a one-prompt change to the attack. Together they stop both bypasses at four articles, but sixteen distorted copies beat them, and they change 29% of clean decisions and discard 39% of the genuine news. Partitioned retrieval also requires control of the retrieval index. Systems that search the open web have no such control and are left with the filter alone. For them, the attack still works.

==> tables/tab_breadth.tex <==
\begin{table*}[t]\centering
\caption{\textbf{One fabricated article on the 308 prediction-market questions, every system and protocol.} Percent, 95\% intervals clustered by question. Protocol~A: the article is placed in the context. Protocol~B: the system retrieves on its own; \emph{article retrieved} is the share of cells in which it did. Single retrieval pools four models (Gemini~3.7 Flash, GPT-5.6, GLM-5.3 Flash, Grok~4.20); the AIA Forecaster pools the three flash models; amplification is 92--100\% in every cell and the 8-draw ensemble matches single retrieval (Table~\ref{tab:believed}). \emph{Price-level}: the 19 questions that ask whether a price will be above a level on a date, a subset of the economic column. Questions per column: 308 / 100 / 104 / 104 / 19; reversal denominators are the opposed cells.}
\label{tab:breadth}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}l ccccc@{}}
\toprule
 & Pooled & Sports & Politics & Economic & Price-level \\
\midrule
\multicolumn{6}{@{}l}{\emph{Single retrieval (hybrid), Protocol A}} \\
\quad Reversal & 74 \ci{69}{79} & 51 \ci{41}{61} & 88 \ci{81}{93} & 83 \ci{76}{89} & 88 \ci{77}{96} \\
\quad Decision flip & 52 \ci{47}{56} & 36 \ci{29}{44} & 67 \ci{59}{74} & 51 \ci{44}{58} & 62 \ci{47}{76} \\
\quad Mean shift toward attacker, pp & 30 \ci{27}{33} & 21 \ci{17}{25} & 43 \ci{38}{48} & 25 \ci{21}{29} & 32 \ci{22}{43} \\
\addlinespace
\multicolumn{6}{@{}l}{\emph{Single retrieval (hybrid), Protocol B}} \\
\quad Reversal & 26 \ci{21}{31} & 16 \ci{9}{23} & 31 \ci{21}{40} & 30 \ci{20}{41} & 8 \ci{0}{21} \\
\quad Decision flip & 20 \ci{16}{24} & 13 \ci{8}{18} & 26 \ci{18}{33} & 21 \ci{15}{28} & 8 \ci{1}{16} \\
\quad Mean shift toward attacker, pp & 9 \ci{7}{12} & 6 \ci{2}{9} & 14 \ci{9}{19} & 8 \ci{5}{11} & 0 \ci{-2}{3} \\
\quad Article retrieved & 28 \ci{23}{33} & 23 \ci{15}{32} & 33 \ci{24}{41} & 28 \ci{19}{37} & 5 \ci{0}{16} \\
\addlinespace
\multicolumn{6}{@{}l}{\emph{AIA Forecaster, Protocol A}} \\
\quad Reversal & 53 \ci{47}{58} & 31 \ci{23}{40} & 63 \ci{54}{72} & 62 \ci{52}{71} & 65 \ci{45}{85} \\
\quad Decision flip & 36 \ci{32}{40} & 21 \ci{15}{27} & 48 \ci{40}{56} & 39 \ci{31}{46} & 53 \ci{33}{72} \\
\quad Mean shift toward attacker, pp & 24 \ci{21}{27} & 12 \ci{9}{15} & 37 \ci{32}{43} & 22 \ci{18}{26} & 34 \ci{24}{44} \\
\addlinespace
\multicolumn{6}{@{}l}{\emph{AIA Forecaster, Protocol B}} \\
\quad Reversal & 45 \ci{40}{51} & 22 \ci{15}{30} & 63 \ci{55}{72} & 46 \ci{36}{56} & 34 \ci{15}{53} \\
\quad Decision flip & 31 \ci{27}{36} & 16 \ci{11}{21} & 48 \ci{41}{57} & 30 \ci{23}{37} & 28 \ci{12}{46} \\
\quad Mean shift toward attacker, pp & 21 \ci{18}{24} & 9 \ci{6}{13} & 37 \ci{32}{43} & 17 \ci{13}{20} & 19 \ci{9}{30} \\
\quad Article retrieved & 92 \ci{89}{94} & 88 \ci{82}{92} & 98 \ci{97}{100} & 89 \ci{84}{94} & 65 \ci{46}{82} \\
\bottomrule
\end{tabular}
\end{table*}

